Enhancing Branch-and-Bound for Multi-Objective 0-1 Programming

In the bi-objective branch-and-bound literature, a key ingredient is objective branching, i.e. to create smaller and disjoint sub-problems in the objective space, obtained from the partial dominance of the lower bound set by the upper bound set. When considering three or more objective functions, however, applying objective branching becomes more complex, and its benefit has so far been unclear. In this paper, we investigate several ingredients which allow to better exploit objective branching in a multi-objective setting. We extend the idea of probing to multiple objectives, enhance it in several ways, and show that when coupled with objective branching, it results in significant speed-ups in terms of CPU times. We also investigate cut generation based on the objective branching constraints. Besides, we generalize the best-bound idea for node selection to multiple objectives and we show that the proposed rules outperform the, in the multi-objective literature, commonly employed depth-first and breadth-first strategies. We also analyze problem specific branching rules. We test the proposed ideas on available benchmark instances for three problem classes with three and four objectives, namely the capacitated facility location problem, the uncapacitated facility location problem, and the knapsack problem. Our enhanced multi-objective branch-and-bound algorithm outperforms the best existing branch-and-bound based approach and is the first to obtain competitive and even slightly better results than a state-of-the-art objective space search method on a subset of the problem classes.

==> tablesExpe/APDXgapRule.tex <==

\begin{tabu} to \linewidth {>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X}
\toprule
p & pb & n & \% CPU update & \# nodes \texttt{BBGAP} & \# nodes \texttt{BBWSN}\\
\midrule
 &  & 65 & 1.8 & 2064.6  (0) & 1278.8  (0)\\

 &  & 230 & 3.9 & 34494.4  (10) & 40765.4  (1)\\

 & \multirow{-3}{*}{\raggedright\arraybackslash CFLP} & 495 & 5.1 & 1918.1  (10) & 4496.5  (10)\\
 
  \cmidrule{2-6}

 &  & 40 & 9.8 & 5826.8  (0) & 7405.8  (0)\\

 &  & 50 & 12.9 & 12459.3  (0) & 14972.0  (0)\\

 &  & 60 & 22.4 & 33760.0  (0) & 43623.0  (0)\\

 &  & 70 & 22.2 & 57832.4  (4) & 105508.2  (0)\\

 & \multirow{-5}{*}{\raggedright\arraybackslash KP} & 80 & 21.1 & 66489.8  (5) & 154884.5  (3)\\

 \cmidrule{2-6}

 &  & 56 & 22.6 & 7524.1  (0) & 12282.8  (0)\\

 &  & 72 & 25.8 & 15755.7  (0) & 26574.4  (0)\\

 &  & 90 & 26.8 & 30022.4  (0) & 52141.6  (0)\\

\multirow{-12}{*}{\raggedleft\arraybackslash 3} & \multirow{-4}{*}{\raggedright\arraybackslash UFLP} & 110 & 34.2 & 17823.2  (10) & 80985.7  (5)\\
\cmidrule{1-6}
 &  & 20 & 8.8 & 923.5  (0) & 1325.6  (0)\\

 &  & 30 & 25.8 & 3640.7  (0) & 5105.6  (0)\\

 & \multirow{-3}{*}{\raggedright\arraybackslash KP} & 40 & 51.0 & 14339.3  (4) & 41642.0  (0)\\

 \cmidrule{2-6}

 &  & 42 & 48.3 & 7984.4  (7) & 22393.8  (0)\\

\multirow{-5}{*}{\raggedleft\arraybackslash 4} & \multirow{-2}{*}{\raggedright\arraybackslash UFLP} & 56 & 50.77 & 350.3  (10) & 39079.1  (10)\\
\bottomrule
\end{tabu}

==> tablesExpe/tabCFLP.tex <==

\begin{tabu} to 1.4\linewidth {>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{CPU} & \multicolumn{2}{c}{\# unsolved} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
n & \texttt{MOF} & \texttt{PS} & \texttt{MOF} & \texttt{PS}\\
\midrule
65 & 10.0 & 6.6 & 0 & 0\\
230 & 1988.0 & 506.5 & 1 & 0\\
495 & 3600.0 & 3600.0 & 10 & 10\\
\bottomrule
\end{tabu}

==> tablesExpe/tabCFLP2.tex <==

\begin{tabu} to \linewidth {>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{2}{c}{CPU} & \multicolumn{2}{c}{\# unsolved} \\
\cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
p & pb & n & avgCpu\_0 & avgCpu\_1 & unsolved\_0 & unsolved\_1\\
\midrule
 &  & 65 & 10.03542 & 12.29319 & 0 & 0\\

 &  & 230 & 1993.33480 & 581.43760 & 1 & 0\\

 & \multirow{-3}{*}{\centering\arraybackslash CFLP} & 495 & 3601.48100 & 3600.63800 & 10 & 10\\

 &  & 56 & 134.12960 & 152.54540 & 0 & 0\\

 &  & 72 & 421.29420 & 473.75870 & 0 & 0\\

 &  & 90 & 1229.19000 & 1334.61400 & 0 & 0\\

\multirow{-7}{*}{\centering\arraybackslash 3} &  & 110 & 3132.80400 & 3188.18500 & 2 & 2\\

\cmidrule{1-7}

 &  & 42 & 306.41380 & 380.56740 & 0 & 0\\

\multirow{-2}{*}{\centering\arraybackslash 4} & \multirow{-6}{*}{\centering\arraybackslash UFLP} & 56 & 3513.76100 & 3573.11500 & 8 & 9\\
\bottomrule
\end{tabu}

==> tablesExpe/tabEnumSep.tex <==

\begin{tabu} to \linewidth {>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X}
\toprule
p & pb & n & \texttt{BB} & \texttt{BB-E}\\
\midrule
 &  & 65 & 10.0 / 6.6 & 10.0 / ?\\

 &  & 230 & 1988.0 / 505.5 & 1993.3 / ?\\

 & \multirow{-3}{*}{\raggedright\arraybackslash CFLP} & 495 & 3600.0 / 3600.0 & 3600.0 / ?\\
 
 \cmidrule{2-5}

 &  & 40 & 46.7 & \textbf{42.5}\\

 &  & 50 & 116.5 & \textbf{108.2}\\

 &  & 60 & 457.8 & \textbf{431.0}\\

 &  & 70 & 1414.1 & \textbf{1341.1}\\

 & \multirow{-5}{*}{\raggedright\arraybackslash KP} & 80 & 2491.5 & \textbf{2388.9} \\
 
 \cmidrule{2-5}

 &  & 56 & 177.3 & \textbf{134.1}\\

 &  & 72 & 564.4 & \textbf{421.3}\\

 &  & 90 & 1590.5 & \textbf{1229.2}\\

\multirow{-12}{*}{\raggedleft\arraybackslash 3} & \multirow{-4}{*}{\raggedright\arraybackslash UFLP} & 110 & 3381.7 & \textbf{3132.8}\\
\cmidrule{1-5}
 &  & 20 & 7.0 & \textbf{2.4}\\

 &  & 30 & 42.0 & \textbf{36.0}\\

 & \multirow{-3}{*}{\raggedright\arraybackslash KP} & 40 & 854.8 & \textbf{751.9}\\

 \cmidrule{2-5}

 &  & 42 & 558.9 & \textbf{306.4}\\

\multirow{-5}{*}{\raggedleft\arraybackslash 4} & \multirow{-2}{*}{\raggedright\arraybackslash UFLP} & 56 & 3600.0 & \textbf{3513.8}\\
\bottomrule
\end{tabu}

==> tablesExpe/tabVarFix.tex <==

\begin{tabular}{r|l|r|l|l|r|r|r}
\hline
p & pb & n & configOB & configVarFix & avgCpu & avgNodes & unsolved\\
\hline
3 & CFLP & 65 & coneOB & mof & 19.701969 & 7906.6 & 0\\
\hline
3 & CFLP & 65 & coneOB & varFix & 15.335203 & 2382.6 & 0\\
\hline
3 & CFLP & 65 & fullOB & mof & 21.896872 & 11786.2 & 0\\
\hline
3 & CFLP & 65 & fullOB & varFix & 10.668681 & 1389.4 & 0\\
\hline
3 & CFLP & 65 & fullOB & varFixDomi & 10.409819 & 1348.4 & 0\\
\hline
3 & CFLP & 65 & noOB & mof & 33.935584 & 15090.4 & 0\\
\hline
3 & CFLP & 65 & noOB & varFix & 65.333300 & 15072.4 & 0\\
\hline
3 & CFLP & 230 & coneOB & mof & 3135.213000 & 198405.7 & 6\\
\hline
3 & CFLP & 230 & coneOB & varFix & 2788.578000 & 65681.8 & 4\\
\hline
3 & CFLP & 230 & fullOB & mof & 3386.505000 & 405597.4 & 7\\
\hline
3 & CFLP & 230 & fullOB & varFix & 2332.705000 & 49365.9 & 1\\
\hline
3 & CFLP & 230 & fullOB & varFixDomi & 2277.704000 & 48679.5 & 1\\
\hline
3 & CFLP & 230 & noOB & mof & 3600.079000 & 78613.1 & 10\\
\hline
3 & CFLP & 230 & noOB & varFix & 3600.098000 & 32593.7 & 10\\
\hline
3 & CFLP & 495 & coneOB & mof & 3600.586000 & 6380.6 & 10\\
\hline
3 & CFLP & 495 & coneOB & varFix & 3600.833000 & 4357.9 & 10\\
\hline
3 & CFLP & 495 & fullOB & mof & 3600.504000 & 33545.9 & 10\\
\hline
3 & CFLP & 495 & fullOB & varFix & 3601.326000 & 4497.9 & 10\\
\hline
3 & CFLP & 495 & fullOB & varFixDomi & 3601.210000 & 4472.2 & 10\\
\hline
3 & CFLP & 495 & noOB & mof & 3600.877000 & 4245.2 & 10\\
\hline
3 & CFLP & 495 & noOB & varFix & 3600.723000 & 2934.4 & 10\\
\hline
3 & KP & 40 & coneOB & mof & 192.925390 & 104268.4 & 0\\
\hline
3 & KP & 40 & coneOB & varFix & 77.736830 & 15918.4 & 0\\
\hline
3 & KP & 40 & fullOB & mof & 200.312350 & 136980.2 & 0\\
\hline
3 & KP & 40 & fullOB & varFix & 65.785170 & 13023.6 & 0\\
\hline
3 & KP & 40 & fullOB & varFixDomi & 64.594820 & 12549.6 & 0\\
\hline
3 & KP & 40 & noOB & mof & 488.185600 & 137544.2 & 0\\
\hline
3 & KP & 40 & noOB & varFix & 366.524400 & 71502.4 & 0\\
\hline
3 & KP & 50 & coneOB & mof & 596.529500 & 283955.0 & 0\\
\hline
3 & KP & 50 & coneOB & varFix & 207.883940 & 34498.6 & 0\\
\hline
3 & KP & 50 & fullOB & mof & 612.702100 & 385177.0 & 0\\
\hline
3 & KP & 50 & fullOB & varFix & 172.348310 & 27261.8 & 0\\
\hline
3 & KP & 50 & fullOB & varFixDomi & 167.676080 & 26110.0 & 0\\
\hline
3 & KP & 50 & noOB & mof & 1811.973900 & 385625.2 & 0\\
\hline
3 & KP & 50 & noOB & varFix & 1190.943700 & 174757.2 & 0\\
\hline
3 & KP & 60 & coneOB & mof & 1971.139300 & 804121.5 & 1\\
\hline
3 & KP & 60 & coneOB & varFix & 873.223800 & 121213.2 & 0\\
\hline
3 & KP & 60 & fullOB & mof & 2000.895600 & 1128878.7 & 2\\
\hline
3 & KP & 60 & fullOB & varFix & 749.723500 & 95023.4 & 0\\
\hline
3 & KP & 60 & fullOB & varFixDomi & 693.918800 & 87230.6 & 0\\
\hline
3 & KP & 60 & noOB & mof & 3523.105000 & 623624.4 & 9\\
\hline
3 & KP & 60 & noOB & varFix & 3369.049000 & 428664.6 & 7\\
\hline
3 & KP & 70 & coneOB & mof & 3324.374000 & 1310720.2 & 7\\
\hline
3 & KP & 70 & coneOB & varFix & 2408.063000 & 289369.3 & 3\\
\hline
3 & KP & 70 & fullOB & mof & 3336.926000 & 1839920.2 & 7\\
\hline
3 & KP & 70 & fullOB & varFix & 2201.654000 & 226918.0 & 2\\
\hline
3 & KP & 70 & fullOB & varFixDomi & 2033.250500 & 208626.0 & 0\\
\hline
3 & KP & 70 & noOB & mof & 3600.080000 & 617265.9 & 10\\
\hline
3 & KP & 70 & noOB & varFix & 3600.067000 & 456791.8 & 10\\
\hline
3 & KP & 80 & coneOB & mof & 3600.173000 & 1368612.3 & 10\\
\hline
3 & KP & 80 & coneOB & varFix & 3314.972000 & 377936.3 & 5\\
\hline
3 & KP & 80 & fullOB & mof & 3600.243000 & 1812818.1 & 10\\
\hline
3 & KP & 80 & fullOB & varFix & 3140.041000 & 303356.0 & 5\\
\hline
3 & KP & 80 & fullOB & varFixDomi & 3048.647000 & 291135.6 & 5\\
\hline
3 & KP & 80 & noOB & mof & 3600.065000 & 499527.9 & 10\\
\hline
3 & KP & 80 & noOB & varFix & 3755.225000 & 367138.9 & 10\\
\hline
3 & UFLP & 56 & coneOB & mof & 234.851800 & 49212.2 & 0\\
\hline
3 & UFLP & 56 & coneOB & varFix & 193.189700 & 20885.2 & 0\\
\hline
3 & UFLP & 56 & fullOB & mof & 451.078900 & 216010.6 & 0\\
\hline
3 & UFLP & 56 & fullOB & varFix & 197.040000 & 14512.6 & 0\\
\hline
3 & UFLP & 56 & fullOB & varFixDomi & 183.463400 & 13263.8 & 0\\
\hline
3 & UFLP & 56 & noOB & mof & 317.000200 & 63239.0 & 0\\
\hline
3 & UFLP & 56 & noOB & varFix & 372.003000 & 62944.2 & 0\\
\hline
3 & UFLP & 72 & coneOB & mof & 768.238800 & 111566.6 & 0\\
\hline
3 & UFLP & 72 & coneOB & varFix & 632.412300 & 47018.2 & 0\\
\hline
3 & UFLP & 72 & fullOB & mof & 1270.105000 & 531514.0 & 0\\
\hline
3 & UFLP & 72 & fullOB & varFix & 677.640000 & 33598.6 & 0\\
\hline
3 & UFLP & 72 & fullOB & varFixDomi & 619.650300 & 29923.0 & 0\\
\hline
3 & UFLP & 72 & noOB & mof & 1093.280900 & 151994.2 & 0\\
\hline
3 & UFLP & 72 & noOB & varFix & 1314.070000 & 151525.4 & 0\\
\hline
3 & UFLP & 90 & coneOB & mof & 1725.473000 & 229470.8 & 0\\
\hline
3 & UFLP & 90 & coneOB & varFix & 1522.061000 & 97638.6 & 0\\
\hline
3 & UFLP & 90 & fullOB & mof & 3509.976000 & 1103596.0 & 5\\
\hline
3 & UFLP & 90 & fullOB & varFix & 1934.348000 & 72544.4 & 0\\
\hline
3 & UFLP & 90 & fullOB & varFixDomi & 1805.700000 & 62457.4 & 0\\
\hline
3 & UFLP & 90 & noOB & mof & 3426.202000 & 275612.6 & 6\\
\hline
3 & UFLP & 90 & noOB & varFix & 3570.748000 & 235776.7 & 9\\
\hline
3 & UFLP & 110 & coneOB & mof & 3600.065000 & 195819.1 & 10\\
\hline
3 & UFLP & 110 & coneOB & varFix & 3438.719000 & 157547.9 & 5\\
\hline
3 & UFLP & 110 & fullOB & mof & 3600.172000 & 681660.1 & 10\\
\hline
3 & UFLP & 110 & fullOB & varFix & 3600.150000 & 73505.6 & 10\\
\hline
3 & UFLP & 110 & fullOB & varFixDomi & 3600.090000 & 72109.6 & 10\\
\hline
3 & UFLP & 110 & noOB & mof & 3600.050000 & 71013.9 & 10\\
\hline
3 & UFLP & 110 & noOB & varFix & 3600.051000 & 72963.3 & 10\\
\hline
4 & KP & 20 & coneOB & mof & 17.606897 & 7651.6 & 0\\
\hline
4 & KP & 20 & coneOB & varFix & 9.799091 & 2103.6 & 0\\
\hline
4 & KP & 20 & fullOB & mof & 17.441911 & 8442.4 & 0\\
\hline
4 & KP & 20 & fullOB & varFix & 8.799238 & 1899.4 & 0\\
\hline
4 & KP & 20 & fullOB & varFixDomi & 8.854886 & 1897.0 & 0\\
\hline
4 & KP & 20 & noOB & mof & 24.623151 & 8998.0 & 0\\
\hline
4 & KP & 20 & noOB & varFix & 20.157051 & 5043.2 & 0\\
\hline
4 & KP & 30 & coneOB & mof & 142.917750 & 43529.8 & 0\\
\hline
4 & KP & 30 & coneOB & varFix & 60.996140 & 8469.2 & 0\\
\hline
4 & KP & 30 & fullOB & mof & 140.549970 & 49641.0 & 0\\
\hline
4 & KP & 30 & fullOB & varFix & 53.943000 & 7589.4 & 0\\
\hline
4 & KP & 30 & fullOB & varFixDomi & 53.680270 & 7572.2 & 0\\
\hline
4 & KP & 30 & noOB & mof & 265.277700 & 53294.2 & 0\\
\hline
4 & KP & 30 & noOB & varFix & 184.016190 & 26693.4 & 0\\
\hline
4 & KP & 40 & coneOB & mof & 1886.156600 & 330758.7 & 2\\
\hline
4 & KP & 40 & coneOB & varFix & 1241.909700 & 82242.8 & 2\\
\hline
4 & KP & 40 & fullOB & mof & 1885.414100 & 430534.1 & 2\\
\hline
4 & KP & 40 & fullOB & varFix & 1137.972500 & 72322.6 & 1\\
\hline
4 & KP & 40 & fullOB & varFixDomi & 1138.185100 & 71908.5 & 1\\
\hline
4 & KP & 40 & noOB & mof & 3078.478200 & 340657.3 & 7\\
\hline
4 & KP & 40 & noOB & varFix & 2467.781000 & 221146.5 & 3\\
\hline
4 & UFLP & 42 & coneOB & mof & 563.031600 & 62617.8 & 0\\
\hline
4 & UFLP & 42 & coneOB & varFix & 547.244100 & 29925.4 & 0\\
\hline
4 & UFLP & 42 & fullOB & mof & 962.677600 & 199163.0 & 0\\
\hline
4 & UFLP & 42 & fullOB & varFix & 489.177400 & 22728.8 & 0\\
\hline
4 & UFLP & 42 & fullOB & varFixDomi & 486.937600 & 22618.8 & 0\\
\hline
4 & UFLP & 42 & noOB & mof & 397.546500 & 68111.2 & 0\\
\hline
4 & UFLP & 42 & noOB & varFix & 602.418500 & 68070.2 & 0\\
\hline
4 & UFLP & 56 & coneOB & mof & 3600.089000 & 71905.0 & 10\\
\hline
4 & UFLP & 56 & coneOB & varFix & 3600.107000 & 49605.7 & 10\\
\hline
4 & UFLP & 56 & fullOB & mof & 3600.077000 & 172122.8 & 10\\
\hline
4 & UFLP & 56 & fullOB & varFix & 3600.197000 & 32013.5 & 10\\
\hline
4 & UFLP & 56 & fullOB & varFixDomi & 3600.135000 & 31985.1 & 10\\
\hline
4 & UFLP & 56 & noOB & mof & 3600.075000 & 183316.4 & 10\\
\hline
4 & UFLP & 56 & noOB & varFix & 3600.065000 & 100648.1 & 10\\
\hline
\end{tabular}

==> tablesExpe/tabVarFix3.tex <==

\begin{tabular}{r|l|r|l|l|r|r|r}
 
p & pb & n & configOB & configVarFix & avgCpu & avgNodes & unsolved\\
 
3 & CFLP & 65 & coneOB & mof & 19.70197 & 7906.6 & 0\\
 
3 & CFLP & 65 & coneOB & varFix & 15.33520 & 2382.6 & 0\\
 
3 & CFLP & 65 & fullOB & mof & 21.89687 & 11786.2 & 0\\
 
3 & CFLP & 65 & fullOB & varFix & 10.66868 & 1389.4 & 0\\
 
3 & CFLP & 65 & fullOB & varFixDomi & 10.40982 & 1348.4 & 0\\
 
3 & CFLP & 65 & noOB & mof & 33.93558 & 15090.4 & 0\\
 
3 & CFLP & 65 & noOB & varFix & 65.33330 & 15072.4 & 0\\
 
3 & CFLP & 230 & coneOB & mof & 3135.21300 & 198405.7 & 6\\
 
3 & CFLP & 230 & coneOB & varFix & 2788.57800 & 65681.8 & 4\\
 
3 & CFLP & 230 & fullOB & mof & 3386.50500 & 405597.4 & 7\\
 
3 & CFLP & 230 & fullOB & varFix & 2332.70500 & 49365.9 & 1\\
 
3 & CFLP & 230 & fullOB & varFixDomi & 2277.70400 & 48679.5 & 1\\
 
3 & CFLP & 230 & noOB & mof & 3600.07900 & 78613.1 & 10\\
 
3 & CFLP & 230 & noOB & varFix & 3600.09800 & 32593.7 & 10\\
 
3 & CFLP & 495 & coneOB & mof & 3600.58600 & 6380.6 & 10\\
 
3 & CFLP & 495 & coneOB & varFix & 3600.83300 & 4357.9 & 10\\
 
3 & CFLP & 495 & fullOB & mof & 3600.50400 & 33545.9 & 10\\
 
3 & CFLP & 495 & fullOB & varFix & 3601.32600 & 4497.9 & 10\\
 
3 & CFLP & 495 & fullOB & varFixDomi & 3601.21000 & 4472.2 & 10\\
 
3 & CFLP & 495 & noOB & mof & 3600.87700 & 4245.2 & 10\\
 
3 & CFLP & 495 & noOB & varFix & 3600.72300 & 2934.4 & 10\\
 
3 & KP & 40 & coneOB & mof & 192.92539 & 104268.4 & 0\\
 
3 & KP & 40 & coneOB & varFix & 77.73683 & 15918.4 & 0\\
 
3 & KP & 40 & fullOB & mof & 200.31235 & 136980.2 & 0\\
 
3 & KP & 40 & fullOB & varFix & 65.78517 & 13023.6 & 0\\
 
3 & KP & 40 & fullOB & varFixDomi & 64.59482 & 12549.6 & 0\\
 
3 & KP & 40 & noOB & mof & 488.18560 & 137544.2 & 0\\
 
3 & KP & 40 & noOB & varFix & 366.52440 & 71502.4 & 0\\
 
3 & KP & 50 & coneOB & mof & 596.52950 & 283955.0 & 0\\
 
3 & KP & 50 & coneOB & varFix & 207.88394 & 34498.6 & 0\\
 
3 & KP & 50 & fullOB & mof & 612.70210 & 385177.0 & 0\\
 
3 & KP & 50 & fullOB & varFix & 172.34831 & 27261.8 & 0\\
 
3 & KP & 50 & fullOB & varFixDomi & 167.67608 & 26110.0 & 0\\
 
3 & KP & 50 & noOB & mof & 1811.97390 & 385625.2 & 0\\
 
3 & KP & 50 & noOB & varFix & 1190.94370 & 174757.2 & 0\\
 
3 & KP & 60 & coneOB & mof & 1971.13930 & 804121.5 & 1\\
 
3 & KP & 60 & coneOB & varFix & 873.22380 & 121213.2 & 0\\
 
3 & KP & 60 & fullOB & mof & 2000.89560 & 1128878.7 & 2\\
 
3 & KP & 60 & fullOB & varFix & 749.72350 & 95023.4 & 0\\
 
3 & KP & 60 & fullOB & varFixDomi & 693.91880 & 87230.6 & 0\\
 
3 & KP & 60 & noOB & mof & 3523.10500 & 623624.4 & 9\\
 
3 & KP & 60 & noOB & varFix & 3369.04900 & 428664.6 & 7\\
 
3 & KP & 70 & coneOB & mof & 3324.37400 & 1310720.2 & 7\\
 
3 & KP & 70 & coneOB & varFix & 2408.06300 & 289369.3 & 3\\
 
3 & KP & 70 & fullOB & mof & 3336.92600 & 1839920.2 & 7\\
 
3 & KP & 70 & fullOB & varFix & 2201.65400 & 226918.0 & 2\\
 
3 & KP & 70 & fullOB & varFixDomi & 2033.25050 & 208626.0 & 0\\
 
3 & KP & 70 & noOB & mof & 3600.08000 & 617265.9 & 10\\
 
3 & KP & 70 & noOB & varFix & 3600.06700 & 456791.8 & 10\\
 
3 & KP & 80 & coneOB & mof & 3600.17300 & 1368612.3 & 10\\
 
3 & KP & 80 & coneOB & varFix & 3314.97200 & 377936.3 & 5\\
 
3 & KP & 80 & fullOB & mof & 3600.24300 & 1812818.1 & 10\\
 
3 & KP & 80 & fullOB & varFix & 3140.04100 & 303356.0 & 5\\
 
3 & KP & 80 & fullOB & varFixDomi & 3048.64700 & 291135.6 & 5\\
 
3 & KP & 80 & noOB & mof & 3600.06500 & 499527.9 & 10\\
 
3 & KP & 80 & noOB & varFix & 3755.22500 & 367138.9 & 10\\
 
3 & UFLP & 56 & coneOB & mof & 234.85180 & 49212.2 & 0\\
 
3 & UFLP & 56 & coneOB & varFix & 193.18970 & 20885.2 & 0\\
 
3 & UFLP & 56 & fullOB & mof & 451.07890 & 216010.6 & 0\\
 
3 & UFLP & 56 & fullOB & varFix & 197.04000 & 14512.6 & 0\\
 
3 & UFLP & 56 & fullOB & varFixDomi & 183.46340 & 13263.8 & 0\\
 
3 & UFLP & 56 & noOB & mof & 317.00020 & 63239.0 & 0\\
 
3 & UFLP & 56 & noOB & varFix & 372.00300 & 62944.2 & 0\\
 
3 & UFLP & 72 & coneOB & mof & 768.23880 & 111566.6 & 0\\
 
3 & UFLP & 72 & coneOB & varFix & 632.41230 & 47018.2 & 0\\
 
3 & UFLP & 72 & fullOB & mof & 1270.10500 & 531514.0 & 0\\
 
3 & UFLP & 72 & fullOB & varFix & 677.64000 & 33598.6 & 0\\
 
3 & UFLP & 72 & fullOB & varFixDomi & 619.65030 & 29923.0 & 0\\
 
3 & UFLP & 72 & noOB & mof & 1093.28090 & 151994.2 & 0\\
 
3 & UFLP & 72 & noOB & varFix & 1314.07000 & 151525.4 & 0\\
 
3 & UFLP & 90 & coneOB & mof & 1725.47300 & 229470.8 & 0\\
 
3 & UFLP & 90 & coneOB & varFix & 1522.06100 & 97638.6 & 0\\
 
3 & UFLP & 90 & fullOB & mof & 3509.97600 & 1103596.0 & 5\\
 
3 & UFLP & 90 & fullOB & varFix & 1934.34800 & 72544.4 & 0\\
 
3 & UFLP & 90 & fullOB & varFixDomi & 1805.70000 & 62457.4 & 0\\
 
3 & UFLP & 90 & noOB & mof & 3426.20200 & 275612.6 & 6\\
 
3 & UFLP & 90 & noOB & varFix & 3570.74800 & 235776.7 & 9\\
 
3 & UFLP & 110 & coneOB & mof & 3600.06500 & 195819.1 & 10\\
 
3 & UFLP & 110 & coneOB & varFix & 3438.71900 & 157547.9 & 5\\
 
3 & UFLP & 110 & fullOB & mof & 3600.17200 & 681660.1 & 10\\
 
3 & UFLP & 110 & fullOB & varFix & 3600.15000 & 73505.6 & 10\\
 
3 & UFLP & 110 & fullOB & varFixDomi & 3600.09000 & 72109.6 & 10\\
 
3 & UFLP & 110 & noOB & mof & 3600.05000 & 71013.9 & 10\\
 
3 & UFLP & 110 & noOB & varFix & 3600.05100 & 72963.3 & 10\\
 
\end{tabular}

==> tablesExpe/tabVarFixCFLP.tex <==

\begin{tabular}{r|l|r|l|l|r|r|r}
\hline
p & pb & n & configOB & configVarFix & avgCpu & avgNodes & unsolved\\
\hline
3 & CFLP & 65 & coneOB & mof & 19.70197 & 7906.6 & 0\\
\hline
3 & CFLP & 65 & coneOB & varFix & 15.33520 & 2382.6 & 0\\
\hline
3 & CFLP & 65 & fullOB & mof & 21.89687 & 11786.2 & 0\\
\hline
3 & CFLP & 65 & fullOB & varFix & 10.66868 & 1389.4 & 0\\
\hline
3 & CFLP & 65 & fullOB & varFixDomi & 10.40982 & 1348.4 & 0\\
\hline
3 & CFLP & 65 & noOB & mof & 33.93558 & 15090.4 & 0\\
\hline
3 & CFLP & 65 & noOB & varFix & 65.33330 & 15072.4 & 0\\
\hline
3 & CFLP & 230 & coneOB & mof & 3135.21300 & 198405.7 & 6\\
\hline
3 & CFLP & 230 & coneOB & varFix & 2788.57800 & 65681.8 & 4\\
\hline
3 & CFLP & 230 & fullOB & mof & 3386.50500 & 405597.4 & 7\\
\hline
3 & CFLP & 230 & fullOB & varFix & 2332.70500 & 49365.9 & 1\\
\hline
3 & CFLP & 230 & fullOB & varFixDomi & 2277.70400 & 48679.5 & 1\\
\hline
3 & CFLP & 230 & noOB & mof & 3600.07900 & 78613.1 & 10\\
\hline
3 & CFLP & 230 & noOB & varFix & 3600.09800 & 32593.7 & 10\\
\hline
3 & CFLP & 495 & coneOB & mof & 3600.58600 & 6380.6 & 10\\
\hline
3 & CFLP & 495 & coneOB & varFix & 3600.83300 & 4357.9 & 10\\
\hline
3 & CFLP & 495 & fullOB & mof & 3600.50400 & 33545.9 & 10\\
\hline
3 & CFLP & 495 & fullOB & varFix & 3601.32600 & 4497.9 & 10\\
\hline
3 & CFLP & 495 & fullOB & varFixDomi & 3601.21000 & 4472.2 & 10\\
\hline
3 & CFLP & 495 & noOB & mof & 3600.87700 & 4245.2 & 10\\
\hline
3 & CFLP & 495 & noOB & varFix & 3600.72300 & 2934.4 & 10\\
\hline
\end{tabular}

==> tablesExpe/tabVarFixCPU.tex <==

\begin{tabular}{r|l|r|r|r|r|r|r|r|r}
\hline
p & pb & n & coneOB - mof & coneOB - varFix & fullOB - mof & fullOB - varFix & fullOB - varFixDomi & noOB - mof & noOB - varFix\\
\hline
3 & CFLP & 65 & 19.70197 & 15.335203 & 21.89687 & 10.668681 & 10.409819 & 33.93558 & 65.33330\\
\hline
3 & CFLP & 230 & 3135.21300 & 2788.578000 & 3386.50500 & 2332.705000 & 2277.704000 & 3600.07900 & 3600.09800\\
\hline
3 & CFLP & 495 & 3600.58600 & 3600.833000 & 3600.50400 & 3601.326000 & 3601.210000 & 3600.87700 & 3600.72300\\
\hline
3 & KP & 40 & 192.92539 & 77.736830 & 200.31235 & 65.785170 & 64.594820 & 488.18560 & 366.52440\\
\hline
3 & KP & 50 & 596.52950 & 207.883940 & 612.70210 & 172.348310 & 167.676080 & 1811.97390 & 1190.94370\\
\hline
3 & KP & 60 & 1971.13930 & 873.223800 & 2000.89560 & 749.723500 & 693.918800 & 3523.10500 & 3369.04900\\
\hline
3 & KP & 70 & 3324.37400 & 2408.063000 & 3336.92600 & 2201.654000 & 2033.250500 & 3600.08000 & 3600.06700\\
\hline
3 & KP & 80 & 3600.17300 & 3314.972000 & 3600.24300 & 3140.041000 & 3048.647000 & 3600.06500 & 3755.22500\\
\hline
3 & UFLP & 56 & 234.85180 & 193.189700 & 451.07890 & 197.040000 & 183.463400 & 317.00020 & 372.00300\\
\hline
3 & UFLP & 72 & 768.23880 & 632.412300 & 1270.10500 & 677.640000 & 619.650300 & 1093.28090 & 1314.07000\\
\hline
3 & UFLP & 90 & 1725.47300 & 1522.061000 & 3509.97600 & 1934.348000 & 1805.700000 & 3426.20200 & 3570.74800\\
\hline
3 & UFLP & 110 & 3600.06500 & 3438.719000 & 3600.17200 & 3600.150000 & 3600.090000 & 3600.05000 & 3600.05100\\
\hline
4 & KP & 20 & 17.60690 & 9.799091 & 17.44191 & 8.799238 & 8.854886 & 24.62315 & 20.15705\\
\hline
4 & KP & 30 & 142.91775 & 60.996140 & 140.54997 & 53.943000 & 53.680270 & 265.27770 & 184.01619\\
\hline
4 & KP & 40 & 1886.15660 & 1241.909700 & 1885.41410 & 1137.972500 & 1138.185100 & 3078.47820 & 2467.78100\\
\hline
4 & UFLP & 42 & 563.03160 & 547.244100 & 962.67760 & 489.177400 & 486.937600 & 397.54650 & 602.41850\\
\hline
4 & UFLP & 56 & 3600.08900 & 3600.107000 & 3600.07700 & 3600.197000 & 3600.135000 & 3600.07500 & 3600.06500\\
\hline
\end{tabular}

==> tablesExpe/tabVarFixKP.tex <==

\begin{tabular}{r|l|r|l|l|r|r|r}
\hline
p & pb & n & configOB & configVarFix & avgCpu & avgNodes & unsolved\\
\hline
3 & KP & 40 & coneOB & mof & 192.925390 & 104268.4 & 0\\
\hline
3 & KP & 40 & coneOB & varFix & 77.736830 & 15918.4 & 0\\
\hline
3 & KP & 40 & fullOB & mof & 200.312350 & 136980.2 & 0\\
\hline
3 & KP & 40 & fullOB & varFix & 65.785170 & 13023.6 & 0\\
\hline
3 & KP & 40 & fullOB & varFixDomi & 64.594820 & 12549.6 & 0\\
\hline
3 & KP & 40 & noOB & mof & 488.185600 & 137544.2 & 0\\
\hline
3 & KP & 40 & noOB & varFix & 366.524400 & 71502.4 & 0\\
\hline
3 & KP & 50 & coneOB & mof & 596.529500 & 283955.0 & 0\\
\hline
3 & KP & 50 & coneOB & varFix & 207.883940 & 34498.6 & 0\\
\hline
3 & KP & 50 & fullOB & mof & 612.702100 & 385177.0 & 0\\
\hline
3 & KP & 50 & fullOB & varFix & 172.348310 & 27261.8 & 0\\
\hline
3 & KP & 50 & fullOB & varFixDomi & 167.676080 & 26110.0 & 0\\
\hline
3 & KP & 50 & noOB & mof & 1811.973900 & 385625.2 & 0\\
\hline
3 & KP & 50 & noOB & varFix & 1190.943700 & 174757.2 & 0\\
\hline
3 & KP & 60 & coneOB & mof & 1971.139300 & 804121.5 & 1\\
\hline
3 & KP & 60 & coneOB & varFix & 873.223800 & 121213.2 & 0\\
\hline
3 & KP & 60 & fullOB & mof & 2000.895600 & 1128878.7 & 2\\
\hline
3 & KP & 60 & fullOB & varFix & 749.723500 & 95023.4 & 0\\
\hline
3 & KP & 60 & fullOB & varFixDomi & 693.918800 & 87230.6 & 0\\
\hline
3 & KP & 60 & noOB & mof & 3523.105000 & 623624.4 & 9\\
\hline
3 & KP & 60 & noOB & varFix & 3369.049000 & 428664.6 & 7\\
\hline
3 & KP & 70 & coneOB & mof & 3324.374000 & 1310720.2 & 7\\
\hline
3 & KP & 70 & coneOB & varFix & 2408.063000 & 289369.3 & 3\\
\hline
3 & KP & 70 & fullOB & mof & 3336.926000 & 1839920.2 & 7\\
\hline
3 & KP & 70 & fullOB & varFix & 2201.654000 & 226918.0 & 2\\
\hline
3 & KP & 70 & fullOB & varFixDomi & 2033.250500 & 208626.0 & 0\\
\hline
3 & KP & 70 & noOB & mof & 3600.080000 & 617265.9 & 10\\
\hline
3 & KP & 70 & noOB & varFix & 3600.067000 & 456791.8 & 10\\
\hline
3 & KP & 80 & coneOB & mof & 3600.173000 & 1368612.3 & 10\\
\hline
3 & KP & 80 & coneOB & varFix & 3314.972000 & 377936.3 & 5\\
\hline
3 & KP & 80 & fullOB & mof & 3600.243000 & 1812818.1 & 10\\
\hline
3 & KP & 80 & fullOB & varFix & 3140.041000 & 303356.0 & 5\\
\hline
3 & KP & 80 & fullOB & varFixDomi & 3048.647000 & 291135.6 & 5\\
\hline
3 & KP & 80 & noOB & mof & 3600.065000 & 499527.9 & 10\\
\hline
3 & KP & 80 & noOB & varFix & 3755.225000 & 367138.9 & 10\\
\hline
4 & KP & 20 & coneOB & mof & 17.606897 & 7651.6 & 0\\
\hline
4 & KP & 20 & coneOB & varFix & 9.799091 & 2103.6 & 0\\
\hline
4 & KP & 20 & fullOB & mof & 17.441911 & 8442.4 & 0\\
\hline
4 & KP & 20 & fullOB & varFix & 8.799238 & 1899.4 & 0\\
\hline
4 & KP & 20 & fullOB & varFixDomi & 8.854886 & 1897.0 & 0\\
\hline
4 & KP & 20 & noOB & mof & 24.623151 & 8998.0 & 0\\
\hline
4 & KP & 20 & noOB & varFix & 20.157051 & 5043.2 & 0\\
\hline
4 & KP & 30 & coneOB & mof & 142.917750 & 43529.8 & 0\\
\hline
4 & KP & 30 & coneOB & varFix & 60.996140 & 8469.2 & 0\\
\hline
4 & KP & 30 & fullOB & mof & 140.549970 & 49641.0 & 0\\
\hline
4 & KP & 30 & fullOB & varFix & 53.943000 & 7589.4 & 0\\
\hline
4 & KP & 30 & fullOB & varFixDomi & 53.680270 & 7572.2 & 0\\
\hline
4 & KP & 30 & noOB & mof & 265.277700 & 53294.2 & 0\\
\hline
4 & KP & 30 & noOB & varFix & 184.016190 & 26693.4 & 0\\
\hline
4 & KP & 40 & coneOB & mof & 1886.156600 & 330758.7 & 2\\
\hline
4 & KP & 40 & coneOB & varFix & 1241.909700 & 82242.8 & 2\\
\hline
4 & KP & 40 & fullOB & mof & 1885.414100 & 430534.1 & 2\\
\hline
4 & KP & 40 & fullOB & varFix & 1137.972500 & 72322.6 & 1\\
\hline
4 & KP & 40 & fullOB & varFixDomi & 1138.185100 & 71908.5 & 1\\
\hline
4 & KP & 40 & noOB & mof & 3078.478200 & 340657.3 & 7\\
\hline
4 & KP & 40 & noOB & varFix & 2467.781000 & 221146.5 & 3\\
\hline
\end{tabular}

==> tablesExpe/tabVarFixUFLP.tex <==

\begin{tabular}{r|l|r|l|l|r|r|r}
\hline
p & pb & n & configOB & configVarFix & avgCpu & avgNodes & unsolved\\
\hline
3 & UFLP & 56 & coneOB & mof & 234.8518 & 49212.2 & 0\\
\hline
3 & UFLP & 56 & coneOB & varFix & 193.1897 & 20885.2 & 0\\
\hline
3 & UFLP & 56 & fullOB & mof & 451.0789 & 216010.6 & 0\\
\hline
3 & UFLP & 56 & fullOB & varFix & 197.0400 & 14512.6 & 0\\
\hline
3 & UFLP & 56 & fullOB & varFixDomi & 183.4634 & 13263.8 & 0\\
\hline
3 & UFLP & 56 & noOB & mof & 317.0002 & 63239.0 & 0\\
\hline
3 & UFLP & 56 & noOB & varFix & 372.0030 & 62944.2 & 0\\
\hline
3 & UFLP & 72 & coneOB & mof & 768.2388 & 111566.6 & 0\\
\hline
3 & UFLP & 72 & coneOB & varFix & 632.4123 & 47018.2 & 0\\
\hline
3 & UFLP & 72 & fullOB & mof & 1270.1050 & 531514.0 & 0\\
\hline
3 & UFLP & 72 & fullOB & varFix & 677.6400 & 33598.6 & 0\\
\hline
3 & UFLP & 72 & fullOB & varFixDomi & 619.6503 & 29923.0 & 0\\
\hline
3 & UFLP & 72 & noOB & mof & 1093.2809 & 151994.2 & 0\\
\hline
3 & UFLP & 72 & noOB & varFix & 1314.0700 & 151525.4 & 0\\
\hline
3 & UFLP & 90 & coneOB & mof & 1725.4730 & 229470.8 & 0\\
\hline
3 & UFLP & 90 & coneOB & varFix & 1522.0610 & 97638.6 & 0\\
\hline
3 & UFLP & 90 & fullOB & mof & 3509.9760 & 1103596.0 & 5\\
\hline
3 & UFLP & 90 & fullOB & varFix & 1934.3480 & 72544.4 & 0\\
\hline
3 & UFLP & 90 & fullOB & varFixDomi & 1805.7000 & 62457.4 & 0\\
\hline
3 & UFLP & 90 & noOB & mof & 3426.2020 & 275612.6 & 6\\
\hline
3 & UFLP & 90 & noOB & varFix & 3570.7480 & 235776.7 & 9\\
\hline
3 & UFLP & 110 & coneOB & mof & 3600.0650 & 195819.1 & 10\\
\hline
3 & UFLP & 110 & coneOB & varFix & 3438.7190 & 157547.9 & 5\\
\hline
3 & UFLP & 110 & fullOB & mof & 3600.1720 & 681660.1 & 10\\
\hline
3 & UFLP & 110 & fullOB & varFix & 3600.1500 & 73505.6 & 10\\
\hline
3 & UFLP & 110 & fullOB & varFixDomi & 3600.0900 & 72109.6 & 10\\
\hline
3 & UFLP & 110 & noOB & mof & 3600.0500 & 71013.9 & 10\\
\hline
3 & UFLP & 110 & noOB & varFix & 3600.0510 & 72963.3 & 10\\
\hline
4 & UFLP & 42 & coneOB & mof & 563.0316 & 62617.8 & 0\\
\hline
4 & UFLP & 42 & coneOB & varFix & 547.2441 & 29925.4 & 0\\
\hline
4 & UFLP & 42 & fullOB & mof & 962.6776 & 199163.0 & 0\\
\hline
4 & UFLP & 42 & fullOB & varFix & 489.1774 & 22728.8 & 0\\
\hline
4 & UFLP & 42 & fullOB & varFixDomi & 486.9376 & 22618.8 & 0\\
\hline
4 & UFLP & 42 & noOB & mof & 397.5465 & 68111.2 & 0\\
\hline
4 & UFLP & 42 & noOB & varFix & 602.4185 & 68070.2 & 0\\
\hline
4 & UFLP & 56 & coneOB & mof & 3600.0890 & 71905.0 & 10\\
\hline
4 & UFLP & 56 & coneOB & varFix & 3600.1070 & 49605.7 & 10\\
\hline
4 & UFLP & 56 & fullOB & mof & 3600.0770 & 172122.8 & 10\\
\hline
4 & UFLP & 56 & fullOB & varFix & 3600.1970 & 32013.5 & 10\\
\hline
4 & UFLP & 56 & fullOB & varFixDomi & 3600.1350 & 31985.1 & 10\\
\hline
4 & UFLP & 56 & noOB & mof & 3600.0750 & 183316.4 & 10\\
\hline
4 & UFLP & 56 & noOB & varFix & 3600.0650 & 100648.1 & 10\\
\hline
\end{tabular}

==> tikzFigures/OB1.tex <==
\begin{center}
\begin{tikzpicture}
            \begin{axis}[axis x line=bottom, axis y line = left, grid=major,
            xmin = 0, xmax = 13,
            ymin = 0, ymax = 10 , ytick={0,1,2,...,10} , xtick = {0,1,2,...,13}]

            % LUB
            \addplot[only marks,mark=square*,red] coordinates {(1,10) (3,9) (5,6) (7,5) (8,3) (9,2) (13,1)};
            % Pts
            \addplot[only marks] coordinates {(1,9) (3,6) (5,5) (7,3) (8,2) (9,1)};

            % LB
            \addplot[thick, samples=100, domain=12:12.7, green,name path = A] {7 - 0.5*x};

            %\addplot[ultra thick,orange] coordinates{(1,9)(3,9)(3,6)};

            \addplot[thick, samples=100, domain=4:7,green,name path = B] {7 - 0.5*x};
            \addplot[thick, samples=100, domain=2:3,green,name path = C] {13 - 2*x};
            \addplot[thick, samples=100, domain=3.5:4,green,name path = D] {13 - 2*x};

            % UB
            \addplot[dashed, samples=100] coordinates{(1,10)(1,9)(3,9)(3,6)(5,6)(5,5)(7,5)(7,3)(8,3)(8,2)(9,2)(9,1)(13,1)};

            % OB
            \addplot[ultra thick,orange] coordinates{(3,6)(7,6)(7,3)};
            %\addplot[ultra thick,orange] coordinates{(9,1)(13,1)};
            
            \addplot[only marks,mark=square*,blue] coordinates {(7,6)};%(3,9) 
            %\addplot[only marks,blue] coordinates {(3,6)};
    
            % domi LB
            \addplot[dotted, thick, samples=100, domain=1.7:2,green] {13 - 2*x};
            \addplot[dotted, thick, samples=100, domain=3:3.5,green] {13 - 2*x};
            \addplot[dotted, thick, samples=100, domain=7:12,green] {7 - 0.5*x};
            
            \path[fill = blue,opacity = 0.15] (0,0) -- (0,6.0) -- (5.0,6.0) -- (5.0,0);
            \path[fill = red,opacity = 0.15] (0,0) -- (0,5.0) -- (7.0,5.0) -- (7.0,0);
            %\path[fill=gray] (35,60) -- (50,60) -- (50,50) -- (70,50) -- (70,35) -- (40,50);
            %\path[fill=gray] (120,10) -- (130,10) -- (130,7) -- (127,7);
    
            \node[] at (5.5,6.5) {$s^1$};
            \node[] at (7.5,5.5) {$s^2$};
            \node[] at (4.5,4.5) {$s^I$};
            \node[] at (7.5,6.5) {$s$};

            \addlegendentry{local UB}
            \addlegendentry{UB set}
            \addlegendentry{LB set}
            %\addlegendentry{OB}

            \end{axis}
            \end{tikzpicture}
                
\end{center}

==> tikzFigures/OB2.tex <==
\begin{center}
    \begin{tikzpicture}
        \begin{axis}[axis x line=bottom, axis y line = left, grid=major,
        xmin = 0, xmax = 13,
        ymin = 0, ymax = 10 , ytick={0,1,2,...,10} , xtick = {0,1,2,...,13}, xlabel = $z_1(x)$, ylabel = $z_2(x)$]

        % LUB
        \addplot[only marks,mark=square*,red] coordinates {(1,10) (3,9) (5,6) (7,5) (8,3) (9,2) (13,1)};
        % Pts
        \addplot[only marks,red,mark=o] coordinates {(1,9) (3,6) (5,5) (7,3) (8,2) (9,1)};

        \addplot[only marks,mark=square*,blue] coordinates {(13,1)};

        % LB
        \addplot[thick, samples=100, domain=12:12.7, green,name path = A] {7 - 0.5*x};
        \addplot[thick, samples=100, domain=4:7,green,name path = B] {7 - 0.5*x};
        \addplot[thick, samples=100, domain=2:3,green,name path = C] {13 - 2*x};
        \addplot[thick, samples=100, domain=3.5:4,green,name path = D] {13 - 2*x};

        \addplot[dotted, thick, samples=100, domain=1.7:2,green] {13 - 2*x};
        \addplot[dotted, thick, samples=100, domain=3:3.5,green] {13 - 2*x};
        \addplot[dotted, thick, samples=100, domain=7:12,green] {7 - 0.5*x};

        % UB
        \addplot[dashed, samples=100] coordinates{(1,10)(1,9)(3,9)(3,6)(5,6)(5,5)(7,5)(7,3)(8,3)(8,2)(9,2)(9,1)(13,1)};

        % Sub-pb
        \path[fill=blue,opacity=0.15] (0,0) -- (0,1.0) -- (13.0,1.0) -- (13.0,0);
        
        \path[fill=blue,opacity=0.15] (0,0) -- (0,6.0) -- (7.0,6.0) -- (7.0,0);
        \addplot[only marks,mark=square*,blue] coordinates {(7,6)};
        
        \path[fill=blue,opacity=0.15] (0,0) -- (0,9.0) -- (3.0,9.0) -- (3.0,0);
        \addplot[only marks,mark=square*,blue] coordinates {(3,9)};
        
        % Search area
        \path[fill=gray,opacity=0.5] (2.0,9.0) -- (3.0,9.0) -- (3.0,7.0);
        \path[fill=gray,opacity=0.5] (3.5,6.0) -- (5.0,6.0) -- (5.0,5.0) -- (7.0,5.0) -- (7.0,3.5) -- (4.0,5.0);
        \path[fill=gray,opacity=0.5] (12.0,1.0) -- (13.0,1.0) -- (13.0,0.65) -- (12.7,0.65);

        \addlegendentry{local UB}
        \addlegendentry{UB set}
        \addlegendentry{SLUBs}
        \addlegendentry{LB set}
    %\addlegendentry{OB}

    \end{axis}
    \end{tikzpicture}
\end{center}

==> unused/sve.tex <==
% #################################
% OB with p > 2
% #################################

\section{Objective branching with $p \geq 3$}

This is what was done in the previous paper. Unfortunately, it is not as trivial as for the bi-objective case to apply objective branching (referred as \emph{full objective branching} in the previous paper). When $p \geq 3$ we compute the sub-problems as follows:

\begin{itemize}
    \item[Step 1.] Compute the local upper bounds that are dominated by the lower bound set. Create the set $\St$, that contains these local upper bounds.
    \item[Step 2.] For any pair of element $(s^1, s^2) \in \St$, compute the ideal point of the pair $s^I$. If $s^I$ is dominated by the lower bound set, we merge $s^1$ and $s^2$ into a super local upper bound $s$, which is the nadir point of $s^1$ and $s^2$. See Figure~\ref{fig:intersectionPoint}.
    \item[Step 3.] Repeat Step 2 until there is no pair with the ideal point dominated by the lower bound set. One sub-problem is created for each element of $\St$. See Figure~\ref{fig:OB}.
\end{itemize}

\begin{figure}
    \centering
    \input{Submission1/tikzFigures/OB1}
    \caption{The ideal point $s^I$ of the local upper bounds $s^1$ and $s^2$ is dominated by the lower bound set. Hence, we merge them into the super local upper bound $s$.}
    \label{fig:intersectionPoint}
\end{figure}

\begin{figure}
    \centering
    \input{Submission1/tikzFigures/OB2}
    \caption{Three sub-problems are created. The objective branching constraints are defined by the SLUBs (Super Local Upper Bounds, blue squares). Note that none of the SLUBs have an ideal point dominated by the lower bound set.}
    \label{fig:OB}
\end{figure}

This is new. In the literature, (full) objective branching works very well when using by itself in the bi-objective case. However, in the three objective case, the benefit is not as large as in the bi-objective case and is even unclear in some cases. For some problem classes, it is better not to use objective branching because the larger number of nodes generated cannot be processed quickly enough. In practice, it was at least as good and sometimes even better to do not apply objective branching, but instead to generate upper bounds on the objective functions, where the upper bounds are defined by the nadir point of the dominated local upper bounds computed in Step~1. This is what was referred as \emph{cone objective branching} in the previous paper, and from this point is the configuration used as the reference for the best known branch-and-bound.


==> unused/talkSophie.tex <==

% #################################
% Variable fixing
% #################################

\section{Variable fixing and branching (old)}

A question that arise from the results from the previous paper is whether it is possible to further exploit the objective branching constraints, given the fact that when used by themselves the results are not as promising as in the bi-objective case. Indeed, we expect solutions that are close to each other in the objective space to be more likely to be similar than solutions that are far from each other. Hence, when objective branching is applied, given the fact that we are in a specific part of the objective space, we would like to identify if possible values that could not be taken by some variables (variable fixing) and meaningful variables to branch on (variable branching).

From now on, we restrict the analysis to problems with binary variables only. Furthermore, experiments are carried out on Knapsack problems (KP), Uncapacitated Facility Location problems (UFLP), and Capacitated Facility Location problems (CFLP) with $3$ objective functions. However, the method can be applied to any number of objectives.

    %\subsection{Variable fixing}
    
    Let $x_i$ be a free variable at node $\eta$ of the branch-and-bound tree. In order to check whether $x_i$ can take value $v \in \{0,1\}$, we solve the linear program $F(i,v) : \min\{0 \ | \ x \in \X^{\eta}, \ x_i = v\}$, where $\X^{\eta}$ is the feasible set of the problem contained in node $\eta$. If $F(i,v)$ is infeasible, we can conclude that $x_i$ cannot take value $v$ in this subproblem. Furthermore, if both $F(i,0)$ and $F(i,1)$ are infeasible, then $x_i$ cannot take an integral value in the subproblem and consequently, the node $\eta$ can be fathomed. To summarize:
    \begin{itemize}
        \item if $F(i,0)$ is infeasible, we fix $x_i$ to 1 and $x_i$ is not free anymore,
        \item if $F(i,1)$ is infeasible, we fix $x_i$ to 0 and $x_i$ is not free anymore,
        \item item if both $F(i,0)$ and $F(i,1)$ are infeasible, the node is fathomed by infeasibility.
    \end{itemize}
    
    Furthermore, if all variable are fixed, the new solution is added to the upper bound set and the node is fathomed by optimality.
    
    In theory, to obtain as much information as possible, one would need to solve $F(i,v)$ for each free variable and each $v \in \{0,1\}$, and repeat the process until no change is observed. Preliminary experiments showed that in practice, this is a very good strategy with respect to the number of nodes, but the large number of linear programs solved significantly worsen the cpu time. A better strategy was to try to fix each free variable to each possible value once, and do not repeat the process. This resulted in slightly larger branching trees, but with much lower cpu times (still not better than the best known configuration at that point though, but close enough (this was the status of the work at the last RAMOO)).
    
    All the cpu time allocated to variable fixing is spent in solving linear programs. Hence, if we are able to reduce the number of linear programs solved, we can improve the total cpu time. For this purpose, one could use pre-processing rules that manually look at the constraints of the problem and check whether some variables cannot take specific values. For instance, for each constraint, one can look at the minimal value of the left-hand side of the constraint and compare that to the right-hand side. Let $I^1$ be the set of variables fixed to $1$ with branching constraints or variable fixing. For a constraint such that $\sum_{i=1}^n a_ix_i \leq b$ where the $a_i$ are all positive, we check whether $\sum_{i\in I^1} = b$. If this condition holds true, then no other variable with a non-negative coefficient in this constraint can take value $1$ and consequently, all such variables are fixed to $0$. Let $x_i$ be such a variable, there is then no need to solve $F(i,1)$ since we already know that $x_i$ cannot take value $1$. In our implementation, we consider additional rules for both equality and inequality constraints, and where both positive and negative coefficients can appear.
    
    Furthermore, one can reduce the cpu time spent in variable fixing by not applying variable fixing in every node. Preliminary experiments showed that on the set of instances considered, very little variable fixing can be applied after the pre-processing rules were applied when no objective branching is used. As a result, we concluded that a good heuristic is to apply variable fixing only when a change in the upper bound of at least one of the objective function is observed compared to the father node, i.e. when we are able to reduce the search region with objective branching.
    
    Another way to avoid solving additional linear programs is to keep track of the last solutions obtained by solving $F$. Indeed, if in this solution we have $x_i = v$, then $F(i,v)$ cannot be infeasible since we already know a solution that is feasible for this program, and thus there is no need to solve it. In our implementation, we keep track of the last solution obtained by solving $F(i,0)$ and of the last solution obtained by solving $F(i,1)$. One can search for feasible solution in the extreme points of the lower bound set as well, but this did not resulted in a significant benefit since as long as we start fixing some variables, the extreme points are more likely to do not be feasible solutions for $F$ anymore.
    
    Finally, a last improvement to variable fixing can be operated by replacing the objective function in $F(i,v)$ by a weighted sum of the objective functions of the initial problem. Hence, the linear program solved becomes $F(i,v,\lambda) : \min\{\lambda Cx \ | \ x \in \X^{\eta}, \ x_i = v\}$. Let $z^*$ be the optimal solution of $F(i,v,\lambda)$, if for any local upper bound $u$ included in the region defined by the objective branching constraint we have $\lambda u \leq z^*$, then we know that the image feasible region of the subproblem where $x_i = v$ is dominated by the upper bound set. This condition is similar to the dominance test used in \cite{StidsenAndersenDammann2014} and \cite{Stidsen18}, and we refer the reader to these reference as for why this is a valid condition. If such a case is detected, then we fix $x_i$ to its opposite value.
    
    The choice of the weight $\lambda$ is an open question. In our implementation, $\lambda$ is set to $(1,...,1)$ after normalizing the objective functions. Preliminary results showed that in practice, adding this dominance rule to the variable fixing scheme was beneficial.
    
    To summarise, the new branching scheme is the following:
    
    \begin{itemize}
        \item[Step 1.] Compute subproblems in the objective space using (full) objective branching.
        \item[Step 2.] If a change is observed in at least one of the objective branching constraints of one of the subproblems, apply variable fixing in each subproblem independently.
        \item[Step 3.] Perform branching on one of the free variables in each subproblems.
    \end{itemize}
    
    Let $x^0$ and $x^1$ be the last optimal solutions obtained from $F(i,0,\lambda)$ and $F(i,1,\lambda)$ respectively, and $\lambda = (1,...,1)$ after normalization of the objective functions, the variable fixing scheme is the following:
    
    \begin{itemize}
        \item[Step 2.1] Try to fix each free variable by using the pre-processing rules. Repeat the process until no change is observed.
        \item[Step 2.2] For each free variable $x_i$ and value $v$, if $x^0_i \ne v$ and $x^1_i \ne v$, solve $F(i,v,\lambda)$.
        \begin{itemize}
            \item If $F(i,0)$ is infeasible or dominated, then $x_i = 1$. Else, update $x^0$.
            \item If $F(i,1)$ is infeasible or dominated, then $x_i = 0$. Else, update $x^1$.
            \item If both $F(i,0)$ and $F(i,1)$ are either infeasible or dominated, fathom the node and exit variable fixing.
        \end{itemize}
        \item[Step 2.3] If all variables were fixed, add the new solution to the upper bound set and fathom the node.
    \end{itemize}
    
    Currently, the choice of the variable to split after variable fixing was performed (Step~3) is an open question. In our implementation, we currently branch on the variable that is the most often fractional among the extreme points included in the search region defined by the new objective branching constraints: If all variables take integer values, we branch on the variable with the average value the closest to $0.5$. Finally, if no extreme point of the lower bound set is included in the new search region, the free variable with the smallest index is chosen.
    
    Preliminary experiments showed that variable fixing is the most beneficial when coupled with full objective branching, both in terms of number of nodes explored and cpu time. Thus, variable fixing is always coupled with full objective branching from this point.
    
    In Figure~\ref{fig:cpu} (see caption for what is what), we can see that variable fixing is clearly beneficial. For each of the problem classes considered, the average cpu time used for solving the instances is significantly reduced. A good explanation for that can be found in Figure~\ref{fig:nodes}, where the average number of nodes explored is depicted. The number of nodes explored is much lower when variable fixing in enabled. However, the gap between the configurations is lower when looking at the cpu time. This suggest that variable fixing come at a cost, and this is observed when looking at the proportion of cpu time spent in variable fixing: $44\%$ in average over all instances considered. But the gain in terms of number of nodes is so huge that variable fixing is significantly beneficial.
    
    \begin{figure}
        \centering
        \includegraphics[width = \textwidth]{Submission1/pngFigures/cpu.png}
        \caption{The average cpu time is given in function of the number of variables. The best known configuration from Section~1 (cone objective branching) is represented by both the green line and the red line. The red one uses a breadth-first for node selection meanwhile the green one uses depth-first. In the blue configuration, variable fixing coupled with full objective branching, presented in Section~2, is added to the framework. The node selection used is the best known, i.e. breadth first for CFLP and UFLP, and depth-first for KP. Finally, the purple line has both variable fixing from Section~2 and the best bound node selection strategy from Section~3.}
        \label{fig:cpu}
    \end{figure}
    
    \begin{figure}
        \centering
        \includegraphics[width = \textwidth]{Submission1/pngFigures/nbNodes.png}
        \caption{The average number of nodes explored is given in function of the number of variables. The best known configuration (cone objective branching) from Section~1 is represented by both the green line and the red line. The red one uses a breadth-first for node selection meanwhile the green one uses depth-first. In the blue configuration, variable fixing coupled with full objective branching, presented in Section~2, is added to the framework. The node selection used is the best known, i.e. breadth first for CFLP and UFLP, and depth-first for KP. Finally, the purple line has both variable fixing from Section~2 and the best bound node selection strategy from Section~3.}
        \label{fig:nodes}
    \end{figure}

\section{Node selection (old)}

Traditionally in the literature, depth-first or breadth-first strategies are used to select the next node to explore \citep{Przybylski17}. However, we can see from Figure~\ref{fig:cpu} that there is no clear winner over all problem classes between the two, and the difference of cpu time can be very large. When developing a generic solver, one does not know in advance what problem class will be solved, and the need for an appropriate node selection rule arise. In this Section, we overcome this difficulty by introducing a best-bound strategy inspired by the single-objective literature.

In order to chose the next node to explore, one needs to define a score to evaluate each node. For this purpose, we propose to simply solve a weighted sum scalarization with weight $\lambda = (1,...,1)$ at each node, and the optimal value of the scalarization becomes the score of the node. Then, the node with the smallest score is selected. This is equivalent to say that we explore next the node that is the most promising in direction $\lambda$. [comment: could we use multiple scores for each node, obtained from multiple weighted sums (obtained for free), and select the score in function of where we have a gap in the objective space. Would that allow us to compare "different weights"? implementation note: can't use heap for finding quickly the best node though]

Preliminary experiments showed that it was beneficial to scale the objective coefficients when considering the $(1,...,1)$ weighted sum as the score. [In our implementation...]

Obtaining the optimal value of the weighted sum does not necessarily imply to resolve a linear program. Indeed, in the linear relaxation, each extreme point is the optimal solution of a weighted sum scalarization \citep{Ehrgott05}. Hence, if the linear relaxation is already computed, one can get the score by searching the extreme point $y$ such that $\lambda y$ is minimal. In order to obtain this information, instead of computing the linear relaxation when the node is selected, we compute the linear relaxation when the node is created. [add more details about why it does not change anything up to dominance test]

In Figure~\ref{fig:cpu}, we can see that the best bound strategy is better than either depth-first or breadth-first in terms of cpu time. Once again, this can be explained by the lower number of nodes explored (see Figure~\ref{fig:nodes}). Another benefit of the best bound strategy is that there is no need anymore to chose between depth-first and breadth-first strategy, assuming that the problem class of the instance solved in known.



\section{Cover cuts (old)}

For any objective in minimization $k$, an objective branching constraint has the form $C^kx \leqq s_k$, where $C^k$ is the vector of coefficients of objective $k$ and $s_k$ the upper bound on objective $k$ resulting from objective space branching. If $C^k$ has positive coefficients only, the objective branching constraint can be seen as a knapsack constraint and thus, cover cuts inequalities can be generated.

The generation of the cuts will be achieved by looking at the pre-image of the extreme points of the lower bound set that satisfy the objective branching constraints. Let $x$ be such an extreme point, i.e. $z(x) \leqq s$, we define the set of variables taking value $1$ in the solution $\mathcal{I}^+ = \{i \in \{1,...,n\} \ | \ x_i = 1\}$; the set of variables taking value $0$ in the solution $\mathcal{I}^- = \{i \in \{1,...,n\} \ | \ x_i = 0\}$; and the set of variables taking a fractional value in the solution $\mathcal{F} = \{i \in \{1,...,n\} \ | \ 0 < x_i < 1\}$. By construction, we have $z_k(x) = \sum_{i\in \Intp} C^k_i + \sum_{i\in \Frac} C^k_ix_i$. Let $f \in \Frac$, we know that since it is fractional, $x_f$ does not take a value that is feasible for the initial problem. Hence, we will test whether any objective constraint is violated in case we set $x_f = 1$ in the current solution (this may violate other constraints as well, but we are interested in the objective branching constraints only here). Indeed, if $C^k_f + \sum_{i \in \Intp} C^k_i > s_k$ for at least one $k \in \{1,...,p\}$, then necessarily the solution becomes infeasible with respect to the objective branching constraint, and at least one of them should take value $0$. Hence, we obtain the cut $\mathcal{C}_f : x_f + \sum_{i \in \Intp} x_i \leq |\Intp|$. Note that $\mathcal{C}_f$ necessarily cuts $x$ out of the feasible set since all variables in $\Intp$ are equal to $1$ and $x_f > 0$.

Let $f,g \in \Frac$, and let $\mathcal{C}_f$ be the cut generated for $x_f$. Using the same principle, the cut $\mathcal{C}_g$ could be generated. However, it is possible to create a stronger cut by trying to lift $\mathcal{C}_f$ using $x_g$. Indeed, if for each objective we consider the $|\Intp|$ smallest coefficients of the variables in $\Intp \cup \{f,g\}$, sum them, and conclude that the threshold $s_k$ is still violated, then the cut $\mathcal{C}_{fg} : x_f + x_g + \sum_{i \in \Intp} x_i \leq |\Intp|$ holds true.

At each node, cover cut inequalities will be generated right after performing objective space branching, i.e. just before variable fixing. That way, variable fixing can benefit from the strengthening of the newly generated objective branching constraints. In particular, we will try to generate cover cuts at each extreme point of the lower bound set $x$ that satisfy the objective branching constraints $z(x) \leqq s$. For each fractional variable $x_f$, $f \in \Frac$, we will try to lift all cover cuts already existing for $x$. If none can be lifted, the cut $\mathcal{C}_f$ is created.












